Weighted quadrature for hierarchical B-splines

We present weighted quadrature for hierarchical B-splines to address the fast formation of system matrices arising from adaptive isogeometric Galerkin methods with suitably graded hierarchical meshes. By exploiting a local tensor-product structure, we extend the construction of weighted rules from the tensor-product to the hierarchical spline setting. The proposed algorithm has a computational cost proportional to the number of degrees of freedom and advantageous properties with increasing spline degree. To illustrate the performance of the method and confirm the theoretical estimates, a selection of 2D and 3D numerical tests is provided.

==> Cost_old.tex <==

%\newcommand{\wtMultivar}[2]{\ensuremath{w^{#1}_{\fnTid{#2},\ptTid{q}}}}
%\newcommand{\wtbMultivar}[2]{\ensuremath{\bar{w}^{#1}_{\fnTid{#2},\ptTid{q}}}}
%\newcommand{\ptbMultivar}[1]{\ensuremath{\bar{\bx}^{#1}_{\ptTid{q}}}}

{\mt

%We fix $\left(\ell,\fnTid{i}\right) \in \dofsHr$, and define $ \mathcal{I}^{(\ell,\fnTid{i})} := \left\lbrace \left(\ell,\fnTid{i}\right) \in \dofsHr \; \vert \; \supp{\fnLvl{\ell}{i}} \cap \supp{\fnLvl{\m}{j}} \neq \emptyset \right\rbrace $.


Following the sum-factorization approach, we exploit $w_{\fnTid{i},\ptTid{q}}^{\mu} = \prod_{s=1}^d w_{s,\fnGid{i}_{s},\ptGid{q}_{s}}^{\mu}$ and $\fnLvl{m}{j}(\ptbMultivar{\mu}) = \prod_{s=1}^{d} \fnUnivar{m}{s,j_s}(\bar{x}_{q_s}^{\mu})$ into equation \eqref{eq:quad_rule} and write it in terms of nested sums:
%
\begin{equation}\label{eq:sumfact}
\begin{aligned} 
\quadrule{\ell}{i} (c \fnLvl{m}{j}) 
& = \sum_{q_1, \ldots, q_d} \prod_{s=1}^d \gs \left ( w_{s,\fnGid{i}_{s},\ptGid{q}_{s}}^{\ell} \fnUnivar{m}{s,j_s}(\bar{x}_{q_s}^{\mu}) \right ) \, \mt c(\bar{x}_{q_1}^{\mu}, \ldots, \bar{x}_{q_d}^{\mu}) \\
& = \sum_{q_d}  w_{d,\fnGid{i}_d,\ptGid{q}_d}^{\ell} \fnUnivar{m}{d,j_d}(\bar{x}_{q_d}^{\mu})
\left( \sum_{q_{d-1}} \ldots \sum_{q_1} w_{1,\fnGid{i}_{1},\ptGid{q}_{1}}^{\ell} \fnUnivar{m}{1,j_1}(\bar{x}_{q_1}^{\mu}) c(\bar{x}_{q_1}^{\mu}, \ldots, \bar{x}_{q_d}^{\mu})\right) 
\end{aligned}
\end{equation}
%
To compute the matrix row corresping to a fixed $\left(\ell,\fnTid{i}\right) \in \dofsHr$, the above expression needs to be evaluated for every $\left(m,\fnTid{j}\right) \in \dofsHr $ such that $\supp{\fnLvl{\ell}{i}} \cap \supp{\fnLvl{\m}{j}} \neq \emptyset$. 

As a preliminary step, for a given level $m$ 
and a given direction $s$, we observe that the number of indices  $j_s$ that must be considered in \eqref{eq:sumfact} is clearly bounded by the number of basis functions of level $m$ whose support intersects the support of $\fnUnivar{\ell}{s,i_s}$. It can be verified that the latter number is bounded by $2p + 1$ when $m \leq \ell$, and by $ \gs 2^{m - \ell} (p+1)+p $ when $m > \ell$. In both cases, since $\mu \geq \max \lbrace m, \ell \rbrace$, this number in turn is bounded by $\gs 2^{\mu - \ell +1} (p + 1)$.

Moreover, if we assume that $\fnLvl{\ell}{i}(\ptbMultivar{\mu})$ does not touch the boundary, we observe that for each direction $s$, the number of index values taken by $q_s$ in the $s$-th sum of \gs  \eqref{eq:sumfact} \mt is roughly $2^{\mu - \ell + 1} (p + 1)$. 

We are now ready to estimate the cost of computing a given matrix row using \eqref{eq:sumfact}. 
We fix $m$, and, as a first step, we evaluate the inner sum for every relevant value of 
%the indices.
$j_1$ and $q_2, \ldots,q_d$. 
Of course in the sum we only need to consider the nonzero terms, and we observe that the term corresponding to a given $q_1$ is nonzero only for the $p+1$ values of the index $j_1$ such that $\fnUnivar{m}{1,j_1}(\bar{x}_{q_1}^{\mu}) \neq 0$.  Moreover, if we preliminary multiply  $w_{1,\fnGid{i}_{1},\ptGid{q}_{1}}^{\ell} \fnUnivar{m}{1,j_1}(\bar{x}_{q_1}^{\mu})$ for all such values of $q_1$ and $j_1$ (which has a negligible cost), each of the nonzero terms adds 2 flops to the cost. 

Since each index $q_1,\ldots,q_d$, can take up to $2^{\mu - \ell + 1} (p + 1)$ values, the cost of the first step is 
\begin{align} \label{eq:cost_inner_sum} 2^{d(\mu - \ell + 1) + 1} \left( p+1 \right)^{d+1} \text{ flops} \end{align}
For $k = 2,\ldots,d$, the $k-$th step of the sum-factorization requires the computation of the sum
%
\begin{align*} \sum_{q_k}  w_{k,\fnGid{i}_k,\ptGid{q}_k}^{\ell} \fnUnivar{m}{k,j_k}(\bar{x}_{q_k}^{\mu}) \left( \sum_{q_1,\ldots,q_{k-1} } \prod_{s=1}^{k-1} w_{s,\fnGid{i}_{s},\ptGid{q}_{s}}^{\ell} \fnUnivar{m}{s,j_s}(\bar{x}_{q_s}^{\mu}) c(\bar{x}_{q_1}^{\mu}, \ldots, \bar{x}_{q_d}^{\mu}) \right) \end{align*}
%
for all values of $j_1, \ldots, j_{k}$ and $q_{k+1}, \ldots, q_d$, where the sum between brackets has already been computed for all the relevant index values. Again we observe that for each value of $q_k$ there are only $p+1$ values of $j_k$ that contribute to the sum, and since the number of values taken by each index $q_{k}, \ldots, q_d$ and $j_1, \ldots, j_{k-1}$ is bounded by $2^{\mu - \ell + 1} (p + 1)$, the cost of this step is again bounded by \eqref{eq:cost_inner_sum}.

In conclusion, if we perform the above computations for every relevant value of $m$, it turns out that the cost to compute the matrix row corresponding to the index $(\ell,\fnTid{i})$ is bounded by
%
\begin{align*}\delta d 2^{d(\mu - \ell + 1) + 1}\left( p+1 \right)^{d+1} \text{ flops}\end{align*}
%
where we introduced the quantity  $\delta = \delta(\ell,\fnTid{i})$, which denotes the number of different function levels that interacts with $\fnLvl{\ell}{i}$.
A bound on the total cost for the matrix assembly can then be obtained by summing over all $(\ell,\fnTid{i}) \in \dofsHr$, which gives
%
\begin{align}\label{eq:total_cost} 2d \left( p+1 \right)^d \sum_{(\ell,\fnTid{i}) \in \dofsHr} \delta 2^{d(\mu - \ell + 1)} \text{ flops} \end{align}

We can derive a more explicit bound on the assembly cost if we observe that $\mu - \ell + 1 \leq r$ and that $\delta \leq 2r - 1$. Hence \eqref{eq:total_cost} is bounded by
\begin{align}\label{eq:total_cost_bound} d (2r-1) 2^{dr + 1} \left( p+1 \right)^{d+1} \ndofsHr = O \left( dr 2^{dr} p^{d+1} \ndofsHr \right) \text{ flops} \end{align}

We observe that the latter expression grows exponentially with respct to the admissibilty parameter $r$, and this effect worsen with the increasing of the dimension $d$.
This might seem unsatisfactory, but we emphasize that \eqref{eq:total_cost_bound} is easily a rather pessimistic bound. Indeed, here we are assuming that every \gs hierarchical B-spline basis function  $\fnLvl{\ell}{i} $, with  $(\ell,\fnTid{i}) \in \dofsHr$, \mt interacts with all the admissible levels. In many practical cases, however, refinement is perfomred only in specific regions of the domain, e.g., \gs in the neighbourhood of \mt  low dimensional manifolds, and as a result the number of basis functions that interact with all the admissible levels is limited.



}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "HB_WQ_paper_draft1"
%%% End:


==> HB_WQ_Algorithms.tex <==

\SetKwProg{Fn}{Function}{ }{end function}
%\SetKwFunction{weightsunivar}{compute\_weights1D\_lvl}
\SetKwFunction{preprocessing}{preprocessing}
\SetKwFunction{aux}{aux\_integrals\_sub\_dim}
\SetKwFunction{assemble}{assemble\_matrix}














%%% Local Variables:
%%% mode: latex
%%% TeX-master: "HB_WQ_paper_draft1"
%%% End:


==> numerical_tests_final/HB_WQ_tests_3D_adm2_dofs_vs_L2error.tex <==
% 0 = n_refinements 
% 1 = id_max_level 
% 2 = n_dofs 
% 3 = n_non_zeros  
% 4 = L2-error     
% 5 = Basis creation (mean)
% 6 = Basis creation (variance)       
% 7 = Basis refinement (mean) 
% 8 = Basis refinement (variance)      
% 9 = Dofs connectivity (mean)    
%10 = Dofs connectivity (variance)      
%11 = WQ-HR creation (mean)         
%12 = WQ-HR creation (variance)         
%13 = Matrix alloc. (mean)
%14 = Matrix alloc. (variance)
%15 = Matrix assembly (mean)    
%16 = Matrix assembly (variance)    
%17 = Matrix alloc.+assembly (mean)  
%18 = Matrix alloc.+assembly (variance)  
%19 = Rhs alloc.+assembly (mean)   
%20 = Rhs alloc.+assembly (variance)   
%21 = Linear system solve (mean)    
%22 = Linear system solve (variance)    
%23 = Time for L2-error (mean)    
%24 = Time for L2-error (variance)    
%25 = Time for output VTK (mean)  
%26 = Time for output VTK (variance)  
%27 = Weights1D computation (mean) 
%28 = Weights1D computation (variance) 
%29 = Eval.pts. definition (mean)    
%30 = Eval.pts. definition (variance)    
%31 = Ids.pts1D support (mean)   
%32 = Ids.pts1D support (variance)   
%33 = Ids.pts1D intersection (mean)  
%34 = Ids.pts1D intersection (variance)  
%35 = Non-TP coefficients (mean)  
%36 = Non-TP coefficients (variance)  
%37 = n_eval_pts


%\pgfplotstableread[skip first n=1]
%{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_2_func_0_beta=0.1_threads_1_adaptive_refinement_wqMat_gaussRHS.dat}\wqdataDegTwo

\pgfplotstableread[skip first n=1]{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_2_func_0_beta=0.1_threads_1_adaptive_refinement_gaussMat_gaussRHS.dat}\gaussdataDegTwo

%\pgfplotstableread[skip first n=1]
%{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_3_func_0_beta=0.1_threads_1_adaptive_refinement_wqMat_gaussRHS.dat}\wqdataDegThree

\pgfplotstableread[skip first n=1]{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_3_func_0_beta=0.1_threads_1_adaptive_refinement_gaussMat_gaussRHS.dat}\gaussdataDegThree

%\pgfplotstableread[skip first n=1]{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_4_func_0_beta=0.1_threads_1_adaptive_refinement_wqMat_gaussRHS.dat}\wqdataDegFour

\pgfplotstableread[skip first n=1]{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_4_func_0_beta=0.1_threads_1_adaptive_refinement_gaussMat_gaussRHS.dat}\gaussdataDegFour

%\pgfplotstableread[skip first n=1]{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_5_func_0_beta=0.1_threads_1_adaptive_refinement_wqMat_gaussRHS.dat}\wqdataDegFive

\pgfplotstableread[skip first n=1]{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_5_func_0_beta=0.1_threads_1_adaptive_refinement_gaussMat_gaussRHS.dat}\gaussdataDegFive

%\pgfplotstableread[skip first n=1]
%{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_6_func_0_beta=0.1_threads_1_adaptive_refinement_wqMat_gaussRHS.dat}\wqdataDegSix

%\pgfplotstableread[skip first n=1]{./numerical_tests_final/time_and_errors_projection_l2_3D_adm_2_degree_6_func_0_beta=0.1_threads_1_adaptive_refinement_gaussMat_gaussRHS.dat}\gaussdataDegSix


\begin{center}

\tikzset{every mark/.append style={scale=0.5}}


%-----------------------------------------------------------------------------------------------
% dofs vs. L2 error --- begin
\begin{figure}[!h]
\begin{tikzpicture}
\begin{loglogaxis}[
    width=\textwidth,
    height=0.7\textwidth,
    title={3D case: DOFs vs. $L^{2}$-error, admissibility $\admissibility=2$.},
    xlabel={$\ndofsHr$},
    ylabel={$L^{2}$-error},
    xmin=9e1,xmax=1e6,
    ymin=9e-7,ymax=3e-1,
    legend pos=south west,
    grid=major
  ]
  % p=2 red
  % p=3 blue
  % p=4 magenta
  % p=5 black
  % p=6 cyan
  
    
  \addplot[red,mark=*]
    table [
      x index=2, % n_dofs
      y index=4% % L2 error
      ] \gaussdataDegTwo;
  \addlegendentry{$p=2$}
        
  \addplot[blue,mark=*]
    table [
      x index=2, % n_dofs
      y index=4% % L2 error
      ] \gaussdataDegThree;
  \addlegendentry{$p=3$}

  \addplot[magenta,mark=*]
    table [
      x index=2, % n_dofs
      y index=4% % L2 error
      ] \gaussdataDegFour;
  \addlegendentry{$p=4$}
        
  \addplot[black,mark=*]
    table [
      x index=2, % n_dofs
      y index=4% % L2 error
      ] \gaussdataDegFive;
  \addlegendentry{$p=5$}
        
%  \addplot[cyan,mark=*]
%    table [
%      x index=2, % n_dofs
%      y index=4% % L2 error
%      ] \gaussdataDegSix;
%   \addlegendentry{$p=6$}


\end{loglogaxis}
\end{tikzpicture}
\caption{DOFs vs. $L^{2}$-error for the 3D case and admissibility parameter $\admissibility=2$. Here is shown the computed $L^{2}$-error using the solution obtained with the standard element-based Gaussian quadrature, because the computed $L^{2}$-error using the solution obtained with hierarchical WQ are nearly identical.}
\label{fig:dofs_vs_err_3D_adm=2}
\end{figure}
% dofs vs. L2 error --- end
%-----------------------------------------------------------------------------------------------
% 
%


\end{center}

